Shadows and headless shadows: a worlds-based, autobiographical approach to reasoning

Many cognitive systems deploy multiple, closed, individually consistent models which can represent interpretations of the present state of the world, moments in the past, possible futures or alternate versions of reality. While they appear under different names, these structures can be grouped under the general term of worlds. The Xapagy architecture is a story-oriented cognitive system which relies exclusively on the autobiographical memory implemented as a raw collection of events organized into world-type structures called {\em scenes}. The system performs reasoning by shadowing current events with events from the autobiography. The shadows are then extrapolated into headless shadows corresponding to predictions, hidden events or inferred relations.

==> RelatedWork.tex <==
% **************************************************
%
%   1 page
%
% **************************************************
\section{Related concepts and comparison}

Worlds have been used as helper concepts to implement reasoning. For instance in SOAR, a substate is created to resolve an impasse.



The Xapagy way to reason with scenes, in contrast is backward looking. Instead of simulating future states of the world, the main way of reasoning is finding scenes in the autobiography of the agent which can be aligned with the current state of the world. 

Before we describe the mechanism in detail, let us make some general observations, of why we believe the Xapagy approach represent a good match of the human abilities. 

There is no doubt that humans use reasoning by simulation. We do have an ability to preview an imagined future, anticipate our actions and the other agents actions in it. All this can be easily recorded at the conscious level. An example of this is the visualization exercises performed by bobsleight pilots before runs.  It is undeniable, however, that at the conscious level, such simulation planning approaches are rare, and alternative endings and/or backtracking is minimal.

In contrast, the explored worlds for emulating DPLL or Gibbs sampling are at least in the dozens, and exponential explosion of combinations is not impossible.

\bigskip

In the architecture we describe, the worlds generated by simulation are replaced by worlds from the autobiographical memory of the agent. Instead of choosing one particular continuation and expectation, the system continually aligns the previous worlds through the mechanisms of shadowing. 

One of the advantages of this model is that there is no need for an internal model of the world, nor models of the other agents. The modeling is based on previous experiences, and it pushes the ``simulation'' to the outside world (for first hand experiences) and to the accuracy of second hand experiences. 

Another advantage is the limited computational complexity. While the possible worlds generated by simulation can be exponentially many in number, the autobiographical references scale linearly with the scale of the autobiography, and, in practice, represent a small subset of it. 

Figure~\ref{fig:Comparison} compared the way in which reasoning about possible futures versus reasoning about applicable pasts work. Note that Xapagy is able to reason about possible futures (see Xapagy paper section). However we argue that the relative frequency of such an activity in a cognitive system should be analogous to those of pre-visualization planning in human life: a relatively rare activity reserved for important events. 

Of course, many of the challenges of reasoning are actually pushing the challenge back to method through which the alignment of the past with the current situation will happen. The mechanism we use is based on the shadowing / headless shadows mechanism. 


\begin{figure}
\begin{center}
\includegraphics[scale=0.4]{figures/PossibleFutures.pdf} 
\includegraphics[scale=0.4]{figures/ApplicablePasts.pdf} 
\label{fig:Comparison}
\caption{Two ways to use worlds in reasoning: possible futures and applicable pasts.}
\end{center}
\end{figure} 


